Uncertainty Quantification for nonparametric regression using Empirical Bayesian neural networks

We propose a new, two-step empirical Bayes-type of approach for neural networks. We show in context of the nonparametric regression model that the procedure (up to a logarithmic factor) provides optimal recovery of the underlying functional parameter of interest and provides Bayesian credible sets with frequentist coverage guarantees. The approach requires fitting the neural network only once, hence it is substantially faster than Bootstrapping type approaches. We demonstrate the applicability of our method over synthetic data, observing good estimation properties and reliable uncertainty quantification.

==> DNNUQMainResult.tex <==
\section{Main result}



Denote $\epsilon_n =  n^{\frac{- \alpha}{2 \alpha + d}}$. 
\begin{thm}\label{thm:main_result}
  Let $\beta, M > 0$. Let $\Pi$ be a prior constucted as in \Cref{Def:Model_sparse}. Let $\mathcal{D}_n = \left( ( X_1, Y_1), \dots, (X_n, Y_n) \right)$.   \begin{itemize}
    \item The posterior contracts at near minimax rate:
      \[
        \limsup_{n \rightarrow \infty}
        \sup_{f_0 \in W^\alpha_M}
        \EE_{f_0}\left(
          \Pi\left(
            f: \| f - f_0 \|_2 \geq M_n \epsilon \log(n)^3
            \middle|
            \mathcal{D}_n
          \right)
        \right)
        = 0,
      \]
      for all $M_n \rightarrow \infty$.
  \end{itemize}
  If in addition the $\alpha$-credible balls $B(c_\alpha, R_\alpha)$ satisfy \Cref{Ass:OptimalApproximation}, then:
  \begin{itemize}
    \item The credible balls have uniform near optimal coverage: There exists $L_{\epsilon, \alpha}$ such that if $B(c_\alpha, R_\alpha)$ is an $\alpha$-credible ball, the ball $B= B(c_\alpha, L_{\epsilon, \alpha} \log(n)^3 R_\alpha)$ satisfies
      \[
        \liminf_n \inf_{f_0 \in W^\beta_{M}([0,1]^d)} \PP_{f_0}^{(n)} (f_0 \in B) \geq 1 - \epsilon \label{eq:UniformCoverageEvenSplitDNN}
      \]
    \item The credible balls have uniform near optimal size:
      \[
        \liminf_n \inf_{f_0 \in W^\beta_{M}([0,1]^d)} \PP_{f_0}^{(n)}(R_\alpha \leq C \epsilon_n) \geq 1- \epsilon
        \label{eq:UniformRadiusEvenSplitDNN}
      \]
      for some large enough $C > 0$.
  \end{itemize}
\end{thm}


==> DNNUQProofEntropy.tex <==
\section{Entropies of Deep neural networks}
Here we collect the results on the entropy of Deep neural networks.

\TODO{Here we write down the results that are relevant for the control of the entropy}
\begin{itemize}
  \item Entropy of sparse DNN
  \item Entropy of Deep DNN
\end{itemize}

\begin{lem}[Lemma 5 in \cite{schmidt-hieber_nonparametric_2017}]
  If $V := \prod_{l=0}^{L+1}(p_\ell + 1)$, then, for any $\delta \ge 0$,
  \[ 
    \log \mathcal{N}( \delta, \mathcal{F}( L, \bf{p}, s, \infty), \| \dot \|_\infty) \leq (s + 1) \log\left( 2 \delta^{-1}(L+1)V^2\right).
  \]
\end{lem}




==> DNNUQProofGenPropDNN.tex <==
\section{Generalization properties of Deep Neural Networks}
Here we collect the properties of Deep neural networks. In particular we prove \Cref{lem:GenPropDNN} here.

\TODO{Here we collect the lemma's that control the generalization properties of DNN}
\begin{itemize}
  \item Main results on generalisation
  \item Controlling generalization error based on entropy conditions
\end{itemize}


\begin{lem}
  Let $0 \le p,q \leq \infty$ and $\beta \ge (1/p - 1/2)_+$ Let $f^0 \in B^\beta_{p,q}([0,1]^d) \cap L^\infty([0,1]^d)$ and $\| f^0 \|_{B^\beta_{p,q}} \leq 1$ and $\| f^0\|_\infty \leq F$, for $F \geq 1$, then, letting $W, L, S, B$ as in \cite{suzuki_adaptivity_2018} Proposition 1, with $N \asymp n^{\frac{d}{2s + d}}$, we obtain
  \[
    \EE_{D_n}[
      \| 
        f^0 - \hat{f} 
      \|_{L^2(P_X)}
    ]
    \lesssim
    n^{- \frac{\beta}{d + 2\beta}} \log(n)^3
  \]
  where $\hat{f}$ is the empirical risk minimizer in the class of near orthogonal, sparse, bounded deep neural networks. In particular, we can write $\hat{f} = \sum_{i = 1}^{k_n} \hat{w}_i \hat{\phi}_i$ where the $\hat{\phi}_i$ are the outputs of the last hidden layer, and weights $\hat{w}_i$ such that the basis functions $(\hat{\phi}_i)_{i = 1}^{k_n}$ are bounded and nearly orthogonal.
\end{lem}

\begin{proof}
  We follow the proof of Theorem 2 in \cite{suzuki_adaptivity_2018}, but then restrict to the class of deep neural networks which are bounded and nearly orthogonal. In order to establish an upperbound on the approximation error we use \Cref{thm:ApproximationPowerBySplines} to establish an upperbound. This still gives the same rates.
\end{proof}



